Domain-specific queries and Web search personalization: some investigations

Major search engines deploy personalized Web results to enhance users' experience, by showing them data supposed to be relevant to their interests. Even if this process may bring benefits to users while browsing, it also raises concerns on the selection of the search results. In particular, users may be unknowingly trapped by search engines in protective information bubbles, called "filter bubbles", which can have the undesired effect of separating users from information that does not fit their preferences. This paper moves from early results on quantification of personalization over Google search query results. Inspired by previous works, we have carried out some experiments consisting of search queries performed by a battery of Google accounts with differently prepared profiles. Matching query results, we quantify the level of personalization, according to topics of the queries and the profile of the accounts. This work reports initial results and it is a first step a for more extensive investigation to measure Web search personalization.

==> eptcsdata.tex <==
\providecommand{\firstpage}{51}
\providecommand{\publicationstatus}{M.H. ter Beek and A. Lluch Lafuente (Eds.): 11th International Workshop\\
on Automated Specification and Verification of Web Systems (WWV'15).\\
EPTCS 188, 2015, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.188.6}{10.4204/EPTCS.188.6}}
\pdfoutput=1

